SMT Queries Decomposition and Caching in Semi-Symbolic Model Checking

In semi-symbolic (control-explicit data-symbolic) model checking the state-space explosion problem is fought by representing sets of states by first-order formulas over the bit-vector theory. In this model checking approach, most of the verification time is spent in an SMT solver on deciding satisfiability of quantified queries, which represent equality of symbolic states. In this paper, we introduce a new scheme for decomposition of symbolic states, which can be used to significantly improve the performance of any semi-symbolic model checker. Using the decomposition, a model checker can issue much simpler and smaller queries to the solver when compared to the original case. Some SMT calls may be even avoided completely, as the satisfaction of some of the simplified formulas can be decided syntactically. Moreover, the decomposition allows for an efficient caching scheme for quantified formulas. To support our theoretical contribution, we show the performance gain of our model checker SymDIVINE on a set of examples from the Software Verification Competition.

==> graphics/Concurrency/lines.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktextfalse
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(3684.00,2834.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(858,440){\makebox(0,0)[r]{\strut{}0.0}}%
      \csname LTb\endcsname%
      \put(858,795){\makebox(0,0)[r]{\strut{}100.0}}%
      \csname LTb\endcsname%
      \put(858,1150){\makebox(0,0)[r]{\strut{}200.0}}%
      \csname LTb\endcsname%
      \put(858,1505){\makebox(0,0)[r]{\strut{}300.0}}%
      \csname LTb\endcsname%
      \put(858,1859){\makebox(0,0)[r]{\strut{}400.0}}%
      \csname LTb\endcsname%
      \put(858,2214){\makebox(0,0)[r]{\strut{}500.0}}%
      \csname LTb\endcsname%
      \put(858,2569){\makebox(0,0)[r]{\strut{}600.0}}%
      \csname LTb\endcsname%
      \put(990,220){\makebox(0,0){\strut{}$0$}}%
      \csname LTb\endcsname%
      \put(1245,220){\makebox(0,0){\strut{}$5$}}%
      \csname LTb\endcsname%
      \put(1500,220){\makebox(0,0){\strut{}$10$}}%
      \csname LTb\endcsname%
      \put(1756,220){\makebox(0,0){\strut{}$15$}}%
      \csname LTb\endcsname%
      \put(2011,220){\makebox(0,0){\strut{}$20$}}%
      \csname LTb\endcsname%
      \put(2266,220){\makebox(0,0){\strut{}$25$}}%
      \csname LTb\endcsname%
      \put(2521,220){\makebox(0,0){\strut{}$30$}}%
      \csname LTb\endcsname%
      \put(2777,220){\makebox(0,0){\strut{}$35$}}%
      \csname LTb\endcsname%
      \put(3032,220){\makebox(0,0){\strut{}$40$}}%
      \csname LTb\endcsname%
      \put(3287,220){\makebox(0,0){\strut{}$45$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(3894,2396){\makebox(0,0)[r]{\strut{}no cache smt no simp}}%
      \csname LTb\endcsname%
      \put(3894,2176){\makebox(0,0)[r]{\strut{}cache smt no simp}}%
      \csname LTb\endcsname%
      \put(3894,1956){\makebox(0,0)[r]{\strut{}no cache part no simp}}%
      \csname LTb\endcsname%
      \put(3894,1736){\makebox(0,0)[r]{\strut{}cache part no simp}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphics/Concurrency/lines}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphics/DeviceDriversLinux64/lines.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktextfalse
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(3684.00,2834.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(858,440){\makebox(0,0)[r]{\strut{}0.0}}%
      \csname LTb\endcsname%
      \put(858,795){\makebox(0,0)[r]{\strut{}100.0}}%
      \csname LTb\endcsname%
      \put(858,1150){\makebox(0,0)[r]{\strut{}200.0}}%
      \csname LTb\endcsname%
      \put(858,1505){\makebox(0,0)[r]{\strut{}300.0}}%
      \csname LTb\endcsname%
      \put(858,1859){\makebox(0,0)[r]{\strut{}400.0}}%
      \csname LTb\endcsname%
      \put(858,2214){\makebox(0,0)[r]{\strut{}500.0}}%
      \csname LTb\endcsname%
      \put(858,2569){\makebox(0,0)[r]{\strut{}600.0}}%
      \csname LTb\endcsname%
      \put(990,220){\makebox(0,0){\strut{}$0$}}%
      \csname LTb\endcsname%
      \put(1220,220){\makebox(0,0){\strut{}$5$}}%
      \csname LTb\endcsname%
      \put(1449,220){\makebox(0,0){\strut{}$10$}}%
      \csname LTb\endcsname%
      \put(1679,220){\makebox(0,0){\strut{}$15$}}%
      \csname LTb\endcsname%
      \put(1909,220){\makebox(0,0){\strut{}$20$}}%
      \csname LTb\endcsname%
      \put(2139,220){\makebox(0,0){\strut{}$25$}}%
      \csname LTb\endcsname%
      \put(2368,220){\makebox(0,0){\strut{}$30$}}%
      \csname LTb\endcsname%
      \put(2598,220){\makebox(0,0){\strut{}$35$}}%
      \csname LTb\endcsname%
      \put(2828,220){\makebox(0,0){\strut{}$40$}}%
      \csname LTb\endcsname%
      \put(3057,220){\makebox(0,0){\strut{}$45$}}%
      \csname LTb\endcsname%
      \put(3287,220){\makebox(0,0){\strut{}$50$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(3894,2396){\makebox(0,0)[r]{\strut{}no cache smt no simp}}%
      \csname LTb\endcsname%
      \put(3894,2176){\makebox(0,0)[r]{\strut{}cache smt no simp}}%
      \csname LTb\endcsname%
      \put(3894,1956){\makebox(0,0)[r]{\strut{}no cache part no simp}}%
      \csname LTb\endcsname%
      \put(3894,1736){\makebox(0,0)[r]{\strut{}cache part no simp}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphics/DeviceDriversLinux64/lines}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphics/ECA/lines.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktextfalse
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(3684.00,2834.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(858,440){\makebox(0,0)[r]{\strut{}0.0}}%
      \csname LTb\endcsname%
      \put(858,795){\makebox(0,0)[r]{\strut{}100.0}}%
      \csname LTb\endcsname%
      \put(858,1150){\makebox(0,0)[r]{\strut{}200.0}}%
      \csname LTb\endcsname%
      \put(858,1505){\makebox(0,0)[r]{\strut{}300.0}}%
      \csname LTb\endcsname%
      \put(858,1859){\makebox(0,0)[r]{\strut{}400.0}}%
      \csname LTb\endcsname%
      \put(858,2214){\makebox(0,0)[r]{\strut{}500.0}}%
      \csname LTb\endcsname%
      \put(858,2569){\makebox(0,0)[r]{\strut{}600.0}}%
      \csname LTb\endcsname%
      \put(990,220){\makebox(0,0){\strut{}$0$}}%
      \csname LTb\endcsname%
      \put(1449,220){\makebox(0,0){\strut{}$50$}}%
      \csname LTb\endcsname%
      \put(1909,220){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%
      \put(2368,220){\makebox(0,0){\strut{}$150$}}%
      \csname LTb\endcsname%
      \put(2828,220){\makebox(0,0){\strut{}$200$}}%
      \csname LTb\endcsname%
      \put(3287,220){\makebox(0,0){\strut{}$250$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(3894,2396){\makebox(0,0)[r]{\strut{}no cache smt no simp}}%
      \csname LTb\endcsname%
      \put(3894,2176){\makebox(0,0)[r]{\strut{}cache smt no simp}}%
      \csname LTb\endcsname%
      \put(3894,1956){\makebox(0,0)[r]{\strut{}no cache part no simp}}%
      \csname LTb\endcsname%
      \put(3894,1736){\makebox(0,0)[r]{\strut{}cache part no simp}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphics/ECA/lines}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphics/ProductLines/lines.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktextfalse
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(3684.00,2834.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(858,440){\makebox(0,0)[r]{\strut{}0.0}}%
      \csname LTb\endcsname%
      \put(858,795){\makebox(0,0)[r]{\strut{}100.0}}%
      \csname LTb\endcsname%
      \put(858,1150){\makebox(0,0)[r]{\strut{}200.0}}%
      \csname LTb\endcsname%
      \put(858,1505){\makebox(0,0)[r]{\strut{}300.0}}%
      \csname LTb\endcsname%
      \put(858,1859){\makebox(0,0)[r]{\strut{}400.0}}%
      \csname LTb\endcsname%
      \put(858,2214){\makebox(0,0)[r]{\strut{}500.0}}%
      \csname LTb\endcsname%
      \put(858,2569){\makebox(0,0)[r]{\strut{}600.0}}%
      \csname LTb\endcsname%
      \put(990,220){\makebox(0,0){\strut{}$0$}}%
      \csname LTb\endcsname%
      \put(1373,220){\makebox(0,0){\strut{}$50$}}%
      \csname LTb\endcsname%
      \put(1756,220){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%
      \put(2139,220){\makebox(0,0){\strut{}$150$}}%
      \csname LTb\endcsname%
      \put(2521,220){\makebox(0,0){\strut{}$200$}}%
      \csname LTb\endcsname%
      \put(2904,220){\makebox(0,0){\strut{}$250$}}%
      \csname LTb\endcsname%
      \put(3287,220){\makebox(0,0){\strut{}$300$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(3894,2396){\makebox(0,0)[r]{\strut{}no cache smt no simp}}%
      \csname LTb\endcsname%
      \put(3894,2176){\makebox(0,0)[r]{\strut{}cache smt no simp}}%
      \csname LTb\endcsname%
      \put(3894,1956){\makebox(0,0)[r]{\strut{}no cache part no simp}}%
      \csname LTb\endcsname%
      \put(3894,1736){\makebox(0,0)[r]{\strut{}cache part no simp}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphics/ProductLines/lines}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphics/Sequentialized/lines.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktextfalse
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(3684.00,2834.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(858,440){\makebox(0,0)[r]{\strut{}0.0}}%
      \csname LTb\endcsname%
      \put(858,795){\makebox(0,0)[r]{\strut{}100.0}}%
      \csname LTb\endcsname%
      \put(858,1150){\makebox(0,0)[r]{\strut{}200.0}}%
      \csname LTb\endcsname%
      \put(858,1505){\makebox(0,0)[r]{\strut{}300.0}}%
      \csname LTb\endcsname%
      \put(858,1859){\makebox(0,0)[r]{\strut{}400.0}}%
      \csname LTb\endcsname%
      \put(858,2214){\makebox(0,0)[r]{\strut{}500.0}}%
      \csname LTb\endcsname%
      \put(858,2569){\makebox(0,0)[r]{\strut{}600.0}}%
      \csname LTb\endcsname%
      \put(990,220){\makebox(0,0){\strut{}$0$}}%
      \csname LTb\endcsname%
      \put(1245,220){\makebox(0,0){\strut{}$5$}}%
      \csname LTb\endcsname%
      \put(1500,220){\makebox(0,0){\strut{}$10$}}%
      \csname LTb\endcsname%
      \put(1756,220){\makebox(0,0){\strut{}$15$}}%
      \csname LTb\endcsname%
      \put(2011,220){\makebox(0,0){\strut{}$20$}}%
      \csname LTb\endcsname%
      \put(2266,220){\makebox(0,0){\strut{}$25$}}%
      \csname LTb\endcsname%
      \put(2521,220){\makebox(0,0){\strut{}$30$}}%
      \csname LTb\endcsname%
      \put(2777,220){\makebox(0,0){\strut{}$35$}}%
      \csname LTb\endcsname%
      \put(3032,220){\makebox(0,0){\strut{}$40$}}%
      \csname LTb\endcsname%
      \put(3287,220){\makebox(0,0){\strut{}$45$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(3894,2396){\makebox(0,0)[r]{\strut{}no cache smt no simp}}%
      \csname LTb\endcsname%
      \put(3894,2176){\makebox(0,0)[r]{\strut{}cache smt no simp}}%
      \csname LTb\endcsname%
      \put(3894,1956){\makebox(0,0)[r]{\strut{}no cache part no simp}}%
      \csname LTb\endcsname%
      \put(3894,1736){\makebox(0,0)[r]{\strut{}cache part no simp}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphics/Sequentialized/lines}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphics/summary/lines.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktextfalse
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(3684.00,2834.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(858,440){\makebox(0,0)[r]{\strut{}0.0}}%
      \csname LTb\endcsname%
      \put(858,795){\makebox(0,0)[r]{\strut{}100.0}}%
      \csname LTb\endcsname%
      \put(858,1150){\makebox(0,0)[r]{\strut{}200.0}}%
      \csname LTb\endcsname%
      \put(858,1505){\makebox(0,0)[r]{\strut{}300.0}}%
      \csname LTb\endcsname%
      \put(858,1859){\makebox(0,0)[r]{\strut{}400.0}}%
      \csname LTb\endcsname%
      \put(858,2214){\makebox(0,0)[r]{\strut{}500.0}}%
      \csname LTb\endcsname%
      \put(858,2569){\makebox(0,0)[r]{\strut{}600.0}}%
      \csname LTb\endcsname%
      \put(990,220){\makebox(0,0){\strut{}$0$}}%
      \csname LTb\endcsname%
      \put(1318,220){\makebox(0,0){\strut{}$100$}}%
      \csname LTb\endcsname%
      \put(1646,220){\makebox(0,0){\strut{}$200$}}%
      \csname LTb\endcsname%
      \put(1974,220){\makebox(0,0){\strut{}$300$}}%
      \csname LTb\endcsname%
      \put(2303,220){\makebox(0,0){\strut{}$400$}}%
      \csname LTb\endcsname%
      \put(2631,220){\makebox(0,0){\strut{}$500$}}%
      \csname LTb\endcsname%
      \put(2959,220){\makebox(0,0){\strut{}$600$}}%
      \csname LTb\endcsname%
      \put(3287,220){\makebox(0,0){\strut{}$700$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(3894,2396){\makebox(0,0)[r]{\strut{}no cache smt no simp}}%
      \csname LTb\endcsname%
      \put(3894,2176){\makebox(0,0)[r]{\strut{}cache smt no simp}}%
      \csname LTb\endcsname%
      \put(3894,1956){\makebox(0,0)[r]{\strut{}no cache part no simp}}%
      \csname LTb\endcsname%
      \put(3894,1736){\makebox(0,0)[r]{\strut{}cache part no simp}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{graphics/summary/lines}}%
    \gplfronttext
  \end{picture}%
\endgroup

